Radar Teach and Repeat: Architecture and Initial Field Testing

Frequency-modulated continuous-wave (FMCW) scanning radar has emerged as an alternative to spinning LiDAR for state estimation on mobile robots. Radar's longer wavelength is less affected by small particulates, providing operational advantages in challenging environments such as dust, smoke, and fog. This paper presents Radar Teach and Repeat (RT&R): a full-stack radar system for long-term off-road robot autonomy. RT&R can drive routes reliably in off-road cluttered areas without any GPS. We benchmark the radar system's closed-loop path-tracking performance and compare it to its 3D LiDAR counterpart. 11.8 km of autonomous driving was completed without interventions using only radar and gyro for navigation. RT&R was evaluated on different routes with progressively less structured scene geometry. RT&R achieved lateral path-tracking root mean squared errors (RMSE) of 5.6 cm, 7.5 cm, and 12.1 cm as the routes became more challenging. On the robot we used for testing, these RMSE values are less than half of the width of one tire (24 cm). These same routes have worst-case errors of 21.7 cm, 24.0 cm, and 43.8 cm. We conclude that radar is a viable alternative to LiDAR for long-term autonomy in challenging off-road scenarios. The implementation of RT&R is open-source and available at: https://github.com/utiasASRL/vtr3.

==> sections/2.literature.tex <==
\section{Related Work}

\subsection{Teach and Repeat}
The Teach and Repeat (T\&R) framework has proven to be effective for localizing and navigating robots in many conditions.
T\&R involves a teaching phase where local submaps are constructed through manual driving, which can then be autonomously repeated \cite{Furgale2010}. 
Due to its simplicity, consistency, and computational efficiency, T\&R has shown its effectiveness using sensors such as stereo vision \cite{Furgale2010} and, more recently, LiDAR sensors \cite{Sehn2023,Burnett2022}. 
The approach's use of local topometric submaps eliminates the need for dense map construction and improves resilience to odometry drift, making T\&R robust, and well-suited to long-term robot autonomy.

% Maybe include a figure
\begin{figure}[htbp]
    \centering
        \centering
        \includegraphics[width=0.8\linewidth]{figures/dummy_t_r_diagram.png}
        \caption{a) A teach path is constructed by compounding relative odometry transformations between vertices in the graph. b) When repeating, localization occurs between poses in the live scan and the map. Compounding localization and odometry allow the red localization prior to be constructed. \sven{I think it makes more sense to have this figure in the methods, rather than in the related work}}
        \label{fig:pose_graph}
\end{figure}

By constructing a topometric pose graph, T\&R retains the ability to achieve metric localization to the path, without needing that estimate to be globally consistent over the whole path. 
As long as the odometry estimates (shown with dotted connections in Figure~\ref{fig:pose_graph} are locally consistent they can be used to construct a prior for localization when repeating.
In Figure~\ref{fig:pose_graph} the dotted red transformation $\check{\Transform{}}_{rm}$ is used as the prior to solve the localization between $\CoordinateFrame{r}$ and $\CoordinateFrame{m}$ for $\hat{\Transform{}}_{rm}$.
The pose graph framework can support any sensor capable of providing odometry and localization. 

\subsection{Sensor Modality Limitations}
\alec{This whole section is vague and unclear. Are we talking about limitations just in T\&R context or everywhere?}
The choice of sensor in localization dictates its efficacy and limitations. Stereo vision, for instance, depends on the presence of consistent and trackable visual features for odometry. Changes in the environment, due to seasonal shifts or weather variations, can disrupt feature matching. Darkness is a failure mode of vision. \alec{You are missing so many citations. At least 4 id say} LiDAR, in contrast, is less affected by lighting variations and can generate detailed point clouds of the surroundings. 
These point clouds are usually merged and downsampled into maps for reference in subsequent navigations. 
The Iterative Closest Point (ICP) algorithm \cite{} is employed to align the map frame with the robot's current position.
LiDAR's extremely dense point cloud data imposes significant computational demands for real-time processing. 
Furthermore, LiDAR systems encounter difficulties in environments filled with smoke, dust particles, snowflakes, or dense vegetation due to the laser beams' inability to penetrate these obstacles, limiting its effectiveness in such conditions \cite{Mielle2019,Ort2020,Cen2018,Courcelle2023}.
\sven{Maybe add one more sentence, explaining why this makes radar attractive - as a better transition to the next section}

%\subsection{Radar Feature Extraction}
%\sven{Is this highly relevant to this paper? Our contributions are not within the choice/method of extraction. I think we can get away with just citing the extractor in our method section}
%Radar's inherent challenges, such as higher noise and lower spatial resolution, complicate feature detection \cite{}. 
%Speckle noise, receiver saturation and multi-path reflection are ubiquitous in radar scan images \cite{hong2020radarslam}. 
%The Constant False Alarm Rate (CFAR) method, a common choice for radar feature detection \cite{rohling2011ordered}, faces issues like redundancy, tuning complexity, and noise-induced false positives. 
%To address these, \cite{alhashimi2021bfar} introduced a Bounded False Alarm Rate (BFAR) that adjusts CFAR's threshold for better accuracy. The resultant extracted point cloud contains vital scene geometry information that can be used for odometry and localization.

\subsection{Radar Odometry and Localization}
Recent studies have suggested that radar is a compelling sensing alternative to LiDAR thanks to its robustness to challenging weather conditions.
Overbye et al. \cite{overbye2023radar} used radar for mapping in off-road navigation, confirming its feasibility for radar-only navigation, obstacle detection and terrain estimation under such conditions. 
A GPU-accelerated Voxel (G-VOM) \cite{???!} Local Mapping system was adopted for mapping to contrast radar maps with LiDAR maps where radar's extended range allows for detecting objects twice as far as LiDAR.
On aerial quadrotors, Michalczyk \cite{michalczyk2023radar} implemented radar-inertial odometry (RIO).
The UAV was moved manually through a dense artificial fog where visual-inertial odometry fails to track useful features in the fog and diverges almost immediately, whereas RIO remains robust and estimates the states successfully despite the fog.  Michalczyk et al. \cite{mielle2019comparative} compared simultaneous localization and mapping (SLAM) performances between LiDAR and radar, finding that radar, despite its lower accuracy in mapping, can still effectively perform SLAM and retain essential map details. 
A full radar-based graph SLAM system was proposed by Hong et al. \cite{hong2020radarslam}
for reliable localization and mapping in large-scale environments with various adverse weather conditions. 
They converted their FMCW radar images to point clouds and estimated radar poses online with keyframe-based pose tracking. Bundle adjustment was performed for local mapping and finally, loop closures were detected using a rotation-invariant global descriptor designed for 3D point clouds. 
They also showed that state-of-the-art vision-based and LiDAR-based SLAM systems failed to finish the testing sequences or drifted quickly due to the severe dynamics in fog, snow and heavy rain \cite{hong2020radarslam}. 
To contend with LiDAR odometry, CFEAR radar odometry has been evolving ever since its introduction in 2021 \cite{Adolfsson2021} where by utilizing the k-strongest return per azimuth filtering technique, a sparse set of oriented surface points were extracted for scan matching. \alec{Runon sentence} 
Subsequent versions including CFEAR-2 \cite{adolfsson2021cfear} and CFEAR-3 \cite{Adolfsson2022}, significantly improved radar odometry by reducing drift, addressing motion distortion, and refining filtering techniques.
CFEAR-3 reported radar localization performance approaching LiDAR SLAM.
Building on CFEAR-3, \cite{frosi2023advancements} proposed a comprehensive radar odometry pipeline consisting of filtering,
motion compensation, oriented surface points computation, smoothing, one-to-many radar scan registration, and pose refinement, setting new benchmarks in radar odometry performance on public radar datasets.
\sven{Need to cite are we ready paper by keenan. We are directly building off of that and that needs to be made clear}

% \subsubsection{\textbf{Radar Datasets}}
% As radar-based localization methods generated promising and robust results, radar datasets have been collected to facilitate the advancement of radar research. The Oxford Radar RobotCar dataset \cite{Barnes2020}, MulRan \cite{Kim2020}, and the Boreas dataset from our lab \cite{Burnett2023} contains all-season driving data in challenging urban weather environments. Most recently, the Oxford Offroad Radar Dataset (OORD) \cite{gadd2024oord} extends \cite{Barnes2020} by providing offroad radar data collected in extreme weather environments with challenging mountainous terrains, such as those in the Scottish highlands.

% \alec{This section seems completely irrelevant. We use none of these and we aren't publishing our data.}

All in all, these studies \alec{Which studies} highlight radar's advantage in disastrous conditions, dense fog or heavy smoke for example. This is where vision and LiDAR typically fail. Most importantly, Burnett et al. \cite{Burnett2022} laid the foundation for a radar-only pipeline that could match the accuracy of a LiDAR-only setup with a considerably smaller map size, highlighting radar's effectiveness and efficiency in localization tasks. This evidence points to radar's viable application in various navigation and mapping contexts, especially in off-road extreme weather settings, presenting a compelling case for its inclusion in this project. \alec{Is this your attempt to say we're building on Keenan's work? This sounds intentionally like we're minimizing the contribution which won't sit well with reviewers. }



==> sections/6.discussion.tex <==
Are the max error locations the same for radar and lidar in each loop.

If so, controller. If not localization

Do the errors decrease as the number of runs increases?
Does the map get updated on every repeat?

Why do we see worse performance?

In a GPS-denied environment, how do we measure quality?

We had no failures in 11.8 km of driving!
What features were critical? Probably gyro
Can we tell from the odometry drift in teaching if there were failure places without enough data.

Are the errors centered around 0? What would a small bias imply?

Do the errors come from localization or odometry?

Are all of the RT\& 

Future work:
Testing in these bad environments
Doppler.
